Stellar Winds on the Main-Sequence II: the Evolution of Rotation and Winds

Aims: We study the evolution of stellar rotation and wind properties for low-mass main-sequence stars. Our aim is to use rotational evolution models to constrain the mass loss rates in stellar winds and to predict how their properties evolve with time on the main-sequence. Methods: We construct a rotational evolution model that is driven by observed rotational distributions of young stellar clusters. Fitting the free parameters in our model allows us to predict how wind mass loss rate depends on stellar mass, radius, and rotation. We couple the results to the wind model developed in Paper I of this series to predict how wind properties evolve on the main-sequence. Results: We estimate that wind mass loss rate scales with stellar parameters as $\dot{M}_\star \propto R_\star^2 \Omega_\star^{1.33} M_\star^{-3.36}$. We estimate that at young ages, the solar wind likely had a mass loss rate that is an order of magnitude higher than that of the current solar wind. This leads to the wind having a higher density at younger ages; however, the magnitude of this change depends strongly on how we scale wind temperature. Due to the spread in rotation rates, young stars show a large range of wind properties at a given age. This spread in wind properties disappears as the stars age. Conclusions: There is a large uncertainty in our knowledge of the evolution of stellar winds on the main-sequence, due both to our lack of knowledge of stellar winds and the large spread in rotation rates at young ages. Given the sensitivity of planetary atmospheres to stellar wind and radiation conditions, these uncertainties can be significant for our understanding of the evolution of planetary environments.

==> Journals.tex <==
\newcommand{\aj}{{AJ}}			
\newcommand{\araa}{{Ann.\ Rev.\ Astron.\ Astrophys.}}		
\newcommand{\apj}{{ApJ}}			
\newcommand{\apjl}{{ApJ Lett.}}		
\newcommand{\apjs}{{ApJS}}		
\newcommand{\apss}{{Ap\&SS}}		
\newcommand{\aap}{{A\&A.}}		
\newcommand{\aapr}{{A\&A~Rev.}}		
\newcommand{\aaps}{{A\&AS}}		
\newcommand{\an}{{AN}}			
\newcommand{\azh}{{AZh}}			
\newcommand{\baas}{{BAAS}}		
\newcommand{\BAIC}{{Bull.\ Astron.\ Inst.\ Czech.}}		
\newcommand{\jrasc}{{JRASC}}		
\newcommand{\memras}{{MmRAS}}		
\newcommand{\mnras}{{MNRAS}}		
\newcommand{\pra}{{Phys.~Rev.~A}}	
\newcommand{\prb}{{Phys.~Rev.~B}}	
\newcommand{\prc}{{Phys.~Rev.~C}}	
\newcommand{\prd}{{Phys.~Rev.~D}}	
\newcommand{\pre}{{Phys.~Rev.~E}}	
\newcommand{\prl}{{Phys.~Rev.~Lett.}}	
\newcommand{\pasp}{{PASP}}		
\newcommand{\pasj}{{PASJ}}		
\newcommand{\qjras}{{QJRAS}}		
\newcommand{\skytel}{{S\&T}}		
\newcommand{\solphys}{{Solar~Phys.}}	
\newcommand{\sovast}{{Soviet~Ast.}}	
\newcommand{\ssr}{{Space~Sci.~Rev.}}	
\newcommand{\zap}{{ZAp}}			
\newcommand{\nat}{{Nature}}		
\newcommand{\iaucirc}{{IAU~Circ.}}
\newcommand{\aplett}{{Astrophys.~Lett.}}
\newcommand{\apspr}{{Astrophys.~Space~Phys.~Res.}}
\newcommand{\bain}{{Bull.~Astron.~Inst.~Netherlands}}
\newcommand{\fcp}{{Fund.~Cosmic~Phys.}}
\newcommand{\gca}{{Geochim.~Cosmochim.~Acta}}
\newcommand{\grl}{{Geophys.~Res.~Lett.}}
\newcommand{\GAFD}{{Geophys.~Astrophys.~Fluid~Dyn.}}
\newcommand{\jcp}{{J.~Chem.~Phys.}}	
\newcommand{\jgr}{{J.~Geophys.~Res.}}	
\newcommand{\jqsrt}{{J.~Quant.~Spec.~Radiat.~Transf.}}
\newcommand{\memsai}{{Mem.~Soc.~Astron.~Italiana}}
\newcommand{\nphysa}{{Nucl.~Phys.~A}}
\newcommand{\physrep}{{Phys.~Rep.}}
\newcommand{\physscr}{{Phys.~Scr}}
\newcommand{\planss}{{Planet.~Space~Sci.}}
\newcommand{\procspie}{{Proc.~SPIE}}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
